VCG Mechanism Design with Unknown Agent Values under Stochastic Bandit Feedback

We study a multi-round welfare-maximising mechanism design problem in instances where agents do not know their values. On each round, a mechanism first assigns an allocation each to a set of agents and charges them a price; at the end of the round, the agents provide (stochastic) feedback to the mechanism for the allocation they received. This setting is motivated by applications in cloud markets and online advertising where an agent may know her value for an allocation only after experiencing it. Therefore, the mechanism needs to explore different allocations for each agent so that it can learn their values, while simultaneously attempting to find the socially optimal set of allocations. Our focus is on truthful and individually rational mechanisms which imitate the classical VCG mechanism in the long run. To that end, we first define three notions of regret for the welfare, the individual utilities of each agent and that of the mechanism. We show that these three terms are interdependent via an $\Omega(T^{\frac{2}{3}})$ lower bound for the maximum of these three terms after $T$ rounds of allocations, and describe an algorithm which essentially achieves this rate. Our framework also provides flexibility to control the pricing scheme so as to trade-off between the agent and seller regrets. Next, we define asymptotic variants for the truthfulness and individual rationality requirements and provide asymptotic rates to quantify the degree to which both properties are satisfied by the proposed algorithm.

==> ancillary_app.tex <==

\section{Some Ancillary Results}
\label{sec:ancillary_app}






==> app_openqs.tex <==

\section{Additional Discussion}
\label{app:openqs}


% This section contains some additional discussion.

% We conclude this paper  with two avenues for future work.



==> broader_impact.tex <==

\section*{Broader Impact}

Mechanism design is an important problem in game theory and has the potential to improve social
welfare and create value across a variety of markets.
However, one of the criticisms levied against mechanism design is that it assumes agents are
sophisticated.
While this might be true for some agents, it is often not the case.
For instance, start ups and small companies need to compete with and rely on larger companies in
cloud
markets, as does the average user who purchases products via e-commerce platforms.
% As a result, the odds are stacked in favour of bigger and sophisticated players who are able to
% discover their preferences on their own, and consequently 
% exert undue influence on a market.
 
We believe the proposed framework enables us to reconsider the way we think about markets in
modern times.
It enables  the application of mechanism design to find welfare
maximising outcomes.
It empowers users by allowing them to discover their preferences by learning
their values, thus making them
strategic participants.
Moreover, the
truthfulness guarantees ensures that no player can manipulate the market to their advantage.

% On the flip side, the ideas can also be used for designing mechanisms that do not aim to maximise
% social welfare. 



==> ee_app.tex <==


\vspace{0.1in}
\subsection{Proof of Theorem~\ref{thm:eemain}}
\label{sec:ee_app}

% In this section, we prove the results for Algorithm~\ref{alg:vcglearn}, when $\estmethod=\estee$.
% In Section~\ref{sec:eewelfare}, we bound the welfare regret.
% In Sections~\ref{sec:eeagentregret}, and~\ref{sec:eesellerregret} we analyze the agent
% and seller regrets respectively for the different choices for $f$ and $g$.
% We combine them
% in Section~\ref{sec:eeagentseller} to prove the second statement of the Theorem.
% Section~\ref{sec:eemaxregret} upper bounds $\EE[\max(n\RT, \RaT, \RmechT)]$.
% Sections~\ref{sec:eerational} and~\ref{sec:eetruthful} establish individual rationality and
% truthfulness to prove the last two statements.
% % We first state a complete version of the theorem which includes all constants.
% Recall that in the first three results, we assume
% that all agents are truthful, while in the last two, we only assume that the relevant agent
% is truthful.
% 
% 
% \vspace{0.1in}
% \subsubsection{Bounding the Welfare Regret: Proof of Theorem~\ref{thm:eemain}.\ref{thm:eewelfare}}
% \label{sec:eewelfare}
% 
% \emph{Proof.}
% We will apply Lemma~\ref{lem:RTgenbound} to control the welfare regret.
% By Lemma~\ref{lem:Etcbound}, we have $\sum_t\PPt(\Etc) \leq 4n$.
% We use the following argument  to bound $\sigmait(\sit)$.
% It uses Lemma~\ref{lem:qTbound}
% and the fact that at time $t$, agent $i$ will have experienced all outcomes $s\in\Scal$
% at least $q_t$ times.
% \begin{align*}
% \sigmait(\sit) = \sigma/\sqrt{\Nit(\sit)} \leq \sigma/\sqrt{q_t} \leq \sqrt{2} K^{1/3} t^{-1/3}.
% \numberthis
% \label{eqn:sigmaitqtbound}
% \end{align*}
% Using Lemma~\ref{lem:subounds} to bound $\sum t^{-\nicefrac{1}{3}}$, we have
% \begin{align*}
% \numberthis
% \label{eqn:eewelfareregbound}
% \EE[\RT] \espleq  4n\Vmax + 3\Vmax K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}
%             +  3\sqrt{2}\betaT n \KotTtt.
% \end{align*}
% The claim follows by substituting for $\betaT$~\eqref{eqn:betat}.
% \qedwhite

% \vspace{0.1in}
% % \subsubsection{Proof of Theorem~\ref{thm:eemain}.\ref{thm:eeagentregret}}
% \subsubsection{Bounding the Agent Regret}
% \label{sec:eeagentregret}
% 
% % In this section, we will bound $\RiT$ for the various choices for $f,g$ when $\estmethod=\estee$.
% 
% % \emph{Proof.}
% We will apply Lemma~\ref{lem:RiTgenbound} and proceed to control the $\at,\bt$ terms
% for the different $f, g$ choices.
% First consider $\at$. 
% % Under $\Et$, $\Valmi(\allocmiopt) \geq \Valmi(\allocmit) \geq \Vlbt(\allocmit)$.
% When $f=\vlb$, we have $\Fmit = \Vlbmit$ and therefore $\EE[\at] = 0$.
% When $f=\vub$, we have $\Fmit = \Vubmit$ and therefore,
% \begin{align*}
% \at \espeq \Vubmit(\allocmit) - \Vlbmit(\allocmit) \espeq \sum_{i=1}^n
% 2\betat\sigmait(\mapfuni(\allocmit)) \;\leq\;
%       2\sqrt{2}\betat n \sigma K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}.
% \end{align*}
% The last step uses an argument similar to~\eqref{eqn:sigmaitqtbound}
%  followed by Lemma~\ref{lem:qTbound}.
% Similarly, when $f=\vbar$, we have
% $\at \leq \Vbarmit(\allocmit) - \Vlbmit(\allocmit) \leq
% \sqrt{2}\betaT n \sigma K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}$.
% Along with Lemma~\ref{lem:subounds}, we have the following bounds on the sum of $\at$'s:
% \begin{align*}
% \numberthis
% \label{eqn:atagent}
% \sum_{t\notin\Expl} \EE[\at|\Et] \,\leq\;
%     \begin{cases}
%         \;0 &\text{if $f=\vlb$}, \\
%         \;\frac{3}{\sqrt{2}}\betaT n \sigma K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}} 
%             \hspace{0.2in}&\text{if $f=\vbar$}, \\
%         \;3\sqrt{2}\betaT n \sigma K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}} 
%             \hspace{0.2in}&\text{if $f=\vub$}.
%     \end{cases}
% \end{align*}
% Now consider $\bt$ and assume the agent participates by rewards.
% When $g=\vub$, $\git=\vubit$ and $\Gmit=\Vubmit$.
% We therefore have,
% $\bt = \vubit(\sit) - \vlbit(\sit) = 2\betat\sigmait(\sit)
% \leq 2\sqrt{2}\sigma \betat \Kottmot$.
% When $g=\vlb$, $\git=\vlbit$ and $\Gmit=\Vlbmit$, which results in
% $\bt= \Vubt(\alloct) - \Vlbt(\alloct) = 2\betat\sum_i\sigmait(\alloct)
% \leq 2\sqrt{2}\sigma \betat n \Kottmot$.
% Similarly, when $g=\vbar$, 
% $\bt \leq \sqrt{2}\betat (n+1) \Kottmot$.
% The above results along with~\eqref{eqn:RiTbound} will give us bounds for the agent regret
% when she participates by rewards.
% % Combining the above with~\eqref{eqn:eeRiTbound} yields the cliam for an agent playing
% % by rewards.
% 
% For an agent participating by bids $\vlbit = \git = \vali$.
% The only change in the analysis is that now $\bt = \Vubt(\alloct) - \Gt(\alloct)$ which
% can be bound in a similar fashion to above.
% % 
% Accounting for these considerations, and using
% Lemma~\ref{lem:subounds}, we have the following bounds on the sum of $\bt$'s:
% \begin{align*}
% \numberthis
% \label{eqn:btagent}
% \sum_{t\notin\Expl} \EE[\bt|\Et] \,\leq\;
%     \begin{cases}
%         \;3\sqrt{2}\betaT \sigma n K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}} 
%             \hspace{0.2in}&\text{if $g=\vlb$}, \\
%         \;\frac{3}{\sqrt{2}}\betaT \sigma (n+\kappaiv) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}} 
%             \hspace{0.2in}&\text{if $g=\vbar$}, \\
%         \;3\sqrt{2}\betaT \sigma \kappaiv K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}} 
%             \hspace{0.2in}&\text{if $g=\vub$}.
%     \end{cases}
% \end{align*}
% Recall that $\kappaiv=1$ if the agent participates by rewards and $0$ if she participates by bids.
% We will use these results to obtain bounds for the agent regret
% in Section~\ref{sec:eeagentseller}.
% % Observe that
% % when $g=\vlb$, there is an additional factor $n$.
% % Therefore, the bounds in~\eqref{eqn:btagent} still hold, although some improvements are possible.
% % For instance, when $g=\vub$, the bound is $0$.
% % We will state this explicitly in Section~\ref{sec:eeagentseller}.
% % becomes $\EE[\rit] \leq \EE[\At|\Et] + \PP(\Etc)$.
% % This translates to a bound on $\RiT$ which is the same as~\eqref{eqn:eeRiTbound} but without
% % the third $3\sqrt{2}\betaT\sigma K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}$ term.
% % The rest of the proof follows along similar lines.
% % \qedwhite

% \vspace{0.1in}
% % \subsubsection{Proof of Theorem~\ref{thm:eemain}.\ref{thm:eemechregret}}
% \subsubsection{Bounding the Seller Regret}
% \label{sec:eemechregret}
% \label{sec:eesellerregret}
% 
% % \emph{Proof.}
% We will apply Lemma~\ref{lem:RmechTgenbound} and control the $\Amit, \Bt$ terms for the
% different choices of $f$ and $g$.
% First consider the $\Amit$ terms.
% When $f=\vub$, then $\Fmit=\Vubmit$ is an upper bound for $\Valmi$ under $\Et$.
% Hence, $\Amit = \max\Valmi - \max\Vubmit \leq 0$.
% When $f=\vlb$, under $\Et$, we obtain the following uniform bound on
% $\Valmi(\alloc) - \Fmit(\alloc)$:
% \begin{align*}
% \forall\alloc\in\Alloc, \;
% \Valmi(\alloc) - \Fmit(\alloc)
% &\leq \Vubmit(\alloc) - \Vlbmit(\alloc) =
% \sum_{j\neq i} 2\betat\sigmajt(\mapfunj(\alloc)) 
% \\
% &\leq 2\sqrt{2}\sigma\betat (n-1) K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}.
% \label{eqn:Amituniformbound}
% \numberthis
% \end{align*}
% Here, the last step uses an argument similar to~\eqref{eqn:sigmaitqtbound}.
% Hence, by  Lemma~\ref{lem:boundmax}, we have
% $\Amit = \max \Valmi - \max \Fmit
% \leq 2\sqrt{2}\sigma\betat (n-1) K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}$.
% When $f=\vbar$, by a similar argument, we have
% $\Amit \leq \sqrt{2}\sigma\betat (n-1) K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}$.
% Along with Lemma~\ref{lem:subounds}, we obtain the following.
% \begin{align*}
% \label{eqn:Atmech}
% \numberthis
% \sum_{i=1}^n \sum_{t\notin\Expl} \EE[\Amit|\Et] \espleq
%     \begin{cases}
%         \;3\sqrt{2}\sigma\betaT n(n-1) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}} 
%         \hspace{0.2in} &\text{if $f=\vlb$}, \\
%         \;\frac{3}{\sqrt{2}}\sigma\betaT n(n-1) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}} 
%         \hspace{0.2in} &\text{if $f=\vbar$}, \\
%         \;0 &\text{if $f=\vub$}.
%     \end{cases}
% \end{align*}
% Now, we turn to $\Bt$.
% For this, note that under $\Et$, $\Val(\allocopt) \geq \Val(\alloct) \geq \Vlbt(\alloct)$.
% When $g=\vlb$, we have $\Gt=\Vlbt$ and therefore $\Bt \leq 0$.
% When $g=\vub$, we have $\Gt=\Vubt$ and therefore,
% \begin{align*}
% \Bt \;\leq\; \Vubt(\alloct) - \Vlbt(\alloct)
%         \;=\; 2\betat\sum_{i=1}^n\sigmait(\sit)
%         \;\leq\; 2\sqrt{2}\sigma n \betat K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}.
% \end{align*}
% A similar analysis shows
% $\Bt\;\leq\; \sqrt{2}\sigma n \betat K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}$
% when $g=\vbar$ which yield the following bounds for the sum of $\Bt$'s.
% \begin{align*}
% \label{eqn:Btmech}
% \numberthis
% (n-1)\sum_{t\notin\Expl} \EE[\Bt|\Et] \espleq
%     \begin{cases}
%         \;0 &\text{if $g=\vlb$}, \\
%         \;\frac{3}{\sqrt{2}}\sigma\betaT n(n-1) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}} 
%         \hspace{0.2in} &\text{if $g=\vbar$}, \\
%         \;3\sqrt{2}\sigma\betaT n(n-1) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}} 
%         \hspace{0.2in} &\text{if $g=\vub$}.
%     \end{cases}
% \end{align*}


% \vspace{0.1in}
% \subsubsection{Proof of Theorem~\ref{thm:eemain}.\ref{thm:eeagentseller}}
% \label{sec:eeagentseller}
% 
% % We use the analysis in Sections~\ref{sec:eeagentregret} and~\ref{sec:eesellerregret} to 
% % establish Theorem~\ref{thm:eemain}.\ref{thm:eeagentseller}.
% 
% \emph{Proof.}
% The claims simply follow by combining the bounds in~\eqref{eqn:atagent},~\eqref{eqn:btagent},
% and Lemma~\ref{lem:RiTgenbound} for the agent and the bounds
% in~\eqref{eqn:Atmech},~\eqref{eqn:Btmech}, and Lemma~\ref{lem:RmechTgenbound} for the seller.
% % Also observe that $3\sqrt{2}\betaT \leq 10\sqrt{\logST}$.
% When $(f,g) = (\vlb,\vub)$,
% \begin{align*}
%  \EE[\RiT] &\leq
%        4n\Vmax +  \big(3\valiexpl  + 3\sqrt{2}\kappaiv \sigma \betaT \big) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}},
% \\
% % \hspace{0.35in}
%  \EE[\RmechT] &\leq
%        4n\Vmax + \Big(3\Vmax  + 6\sqrt{2}\sigma \betaT n(n-1) \Big) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}.
% \end{align*}
% % Here $\kappaiv=1$ when the agent participates by rewards and $\kappaiv = 0$ when she participates
% % by bids.
% When $(f,g) = (\vub,\vlb)$,
% \begin{align*}
%  \EE[\RiT] &\leq
%        4n\Vmax +  \big(3\valiexpl  + 6\sqrt{2}\sigma \betaT n \,\big) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}},
% \\
% % \hspace{0.65in}
%  \EE[\RmechT] &\leq
%        4n + 3\Vmax K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}.
% \end{align*}
% Finally, when $(f,g) = (\vbar,\vbar)$, we have the bounds below. %$\kappaiv$ is as defined above.
% \begin{align*}
%  \EE[\RiT] &\leq
%        4n +  \big(3\valiexpl  + 3\sqrt{2} \sigma \betaT (n + \kappaiv/2) \big) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}},
% \\
% % \hspace{0.35in}
%  \EE[\RmechT] &\leq
%        4n + \Big(3\Vmax  + 3\sqrt{2}\sigma \betaT n(n-1) \Big) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}.
% \end{align*}
% 
% \vspace{-0.2in}
% \qedwhite


% \vspace{0.1in}
% \subsubsection{Proof of Theorem~\ref{thm:eemain}.\ref{thm:eemaxregret}}
% \label{sec:eemaxregret}
% 
% \emph{Proof.}
% We will use Lemma~\ref{lem:MaxRegretgenbound} to control the maximum of the three regret
% terms.
% We already have a bound on $\RT$ from Section~\ref{sec:eewelfare},
% and bounds on $\Amit, \Bt$ from Section~\ref{sec:eesellerregret}.
% The bounds
% for $-\Amit, -\Bt$ are obtained by simply reversing the argument.
% First consider, $|\Amit|$.
% If $f=\vub$, we already saw $\Amit \leq 0$.
% By using an argument similar to~\eqref{eqn:Amituniformbound}, we obtain
% $-\Amit \leq 2\sqrt{2}\sigma\betat (n-1)\Kottmot$.
% % Therefore, $|\Amit| \leq 2\sqrt{2}\sigma\betat (n-1)\Kottmot$.
% Similarly, if $f=\vlb$, we already saw $\Amit \leq 2\sqrt{2}\sigma\betat (n-1)\Kottmot$.
% Moreover,
% \[
% -\Amit = \Vlbmit(\allocmit) - \Valmi(\allocopt)
% \leq \Valmi(\allocmit) - \Valmi(\allocopt) \leq 0.
% \]
% % Therefore, $|\Amit| \leq 2\sqrt{2}\sigma\betat (n-1)\Kottmot$.
% Finally, when $f=\vbar$,  both $\Amit$ and $-\Amit$ can be 
% bounded by $\sqrt{2}\sigma\betat (n-1)\Kottmot$.
% Therefore,  for all $f$ values we  have $|\Amit| \leq 2\sqrt{2}\sigma\betat (n-1)\Kottmot$.
% After an application of Lemma~\ref{lem:subounds}, we obtain,
% \begin{align*}
% \numberthis
% \label{eqn:Amitmodbound}
% \sum_i\sum_{t\notin\Expl} \EE[|\Amit|\,|\Et] \leq 3\sqrt{2}\sigma\betat n(n-1)\KotTtt.
% \end{align*}
% By following a similar argument, we can obtain
% $(n-1)\sum_{t\notin\Expl}\EE[|\Bt|\,|\Et] \leq 3\sqrt{2}\sigma\betat n(n-1)\KotTtt$.
% % Combining this with~\eqref{eqn:RmechTabsbound}, leads to the bound on $\EE[|\RmechT|]$.
% % \[
% %  \EE[|\RmechT|] \leq
% %        4n + \Big(3\Vmax  + 6\sqrt{2}\sigma \betaT n(n-1) \Big) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}.
% % \]
% The claim follows by combining the above with Lemma~\ref{lem:MaxRegretgenbound},
% the bound on the welfare regret in~\eqref{eqn:eewelfareregbound},
% and Lemma~\ref{lem:Etcbound} to control $\sum_{t\notin\Expl}\PPt(\Etc)$.
% %  and some algebraic manipulations.
% \qedwhite

% \vspace{0.1in}
% \subsubsection{Individual Rationality: Proof of Theorem~\ref{thm:eemain}.\ref{thm:eerational}}
% \label{sec:eerational}
% 
% \emph{Proof.}
% For all agents, $\utilit\geq 0$ when $t\in\Expl$, so let us consider $t\notin\Expl$, where,
% by Fact~\ref{fac:algoutils},
% \begin{align*}
% \numberthis
% \label{eqn:utilitirdecomp}
% \utilit = \underbrace{\vali(\sit) - \git(\sit)}_{\ct} + \underbrace{\Gt(\alloct) -
% \Fmit(\allocmit)}_{\dt}.
% \end{align*}
% % We will first bound $\ct$.
% % If agent $i$ participates by bids truthfully, $\git = \vali$ and hence $\ct=0$.
% % To bound $\ct$ from below when she participates by values, 
% % let $\ctildet = \max(0, \git(\sit) - \vali(\sit))\geq 0$.
% % Clearly, $\ct \geq -\ctildet$.
% % % Now, conditioning on $\Eit$~\eqref{eqn:Etdefn}, we have
% % Observing that  $\vali\leq \vubit$ under $\Eit$~\eqref{eqn:Etdefn}, and that
% % $\sigmait(\sit) \leq \sigma K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}$, we have,
% % \[
% % \EE[\ctildet|\Eit] \leq 0 \hspace{0.05in}\text{if $g=\vlb$},
% % \hspace{0.3in}
% % \EE[\ctildet|\Eit] \leq \sqrt{2}\sigma\betat K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}
% %     \hspace{0.05in}\text{if $g=\vbar$},
% % \hspace{0.3in}
% % \EE[\ctildet|\Eit] \leq 2\sqrt{2}\sigma\betat K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}
% %     \hspace{0.05in}\text{if $g=\vub$}.
% % \]
% We will first bound $\ct$.
% If agent $i$ participates by bids truthfully, $\git = \vali$ and hence $\ct=0$.
% To bound $\ct$ when she participates by rewards truthfully,
% let $\ctildet = \max(0, \git(\sit) - \vali(\sit))\geq 0$.
% Clearly, $\ct \geq -\ctildet$.
% % Now, conditioning on $\Eit$~\eqref{eqn:Eitdefn}, we have
% Observing that  $\vali\leq \vubit$ under $\Eit$~\eqref{eqn:Etdefn}, we have,
% \[
% \EE[\ctildet|\Eit] \leq 0 \hspace{0.10in}\text{if $g=\vlb$},
% % \hspace{0.3in}
% % \EE[\ctildet|\Eit] \leq \betat \sigmait(\sit)
% %     \hspace{0.05in}\text{if $g=\vbar$},
% \hspace{0.2in}
% \EE[\ctildet|\Eit] \leq \betat \sigmait(\sit)
%     \hspace{0.10in}\text{if $g=\vbar$}.
% \hspace{0.2in}
% \EE[\ctildet|\Eit] \leq 2 \betat \sigmait(\sit)
%     \hspace{0.10in}\text{if $g=\vub$}.
% \]
% % 
% % If she participates by rewards, 
% % $\EE[\vbarit(s)] = \vali(s)$ since $\Nit(s)$
% % % the number of times agent $i$ has experienced outcome $s$ in the first $t-1$ rounds,
% % is a deterministic quantity.
% % % 
% % % let $\ctildet = \max(0, \git(\sit) - \vali(\sit))\geq 0$.
% % % Clearly, $\ct \geq -\ctildet$.
% % % % Now, conditioning on $\Eit$~\eqref{eqn:Etdefn}, we have
% % Observing that $\sigmait(\sit) \leq \sigma K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}$, we have,
% % \[
% % \EE[\ct] = \betat\sigmait(\sit) > 0 \hspace{0.05in}\text{if $g=\vlb$},
% % \hspace{0.3in}
% % \EE[\ct] = 0
% %     \hspace{0.05in}\text{if $g=\vbar$},
% % \hspace{0.3in}
% % \EE[\ct]  = -\betat\sigmait(\sit) \geq -2\sqrt{2}\sigma\betat K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}
% %     \hspace{0.05in}\text{if $g=\vub$}.
% % \]
% % % therefore
% To bound $\dt$,
%  observe that when $\estmethod=\estee$,
% $\vlbit, \vbarit, \vubit$ are vertically shifted functions;
% for agents participating by bids, they are identical while for agents participating by rewards,
%  we use only one observation per allocation
% per agent in each exploration phase.
% Therefore,
% $\Vlbt, \Vbart, \Vubt$ are also vertically shifted functions and hence
%  $\alloct = \argmax\Vubt = \argmax\Vlbt = \argmax\Vbart$.
% First consider the case $(f,g) = (\vbar,\vbar)$.
% Since, $\Vbart = \Vbarmit + \vbarit$ and $\vbarit\geq 0$ (recall from~\eqref{eqn:learnterms}
% that we clip $\vbarit$ between $0$ and $1$),
% we have that  $\Vbart \geq \Vbarmit$.
% Therefore, $\dt = \max\Vbart - \max \Vbarmit \geq 0$.
% By a similar argument, when $(f,g) = (\vlb,\vub)$,
% $\dt = \max\Vubt - \max \Vlbmit \geq \max\Vubt - \max\Vubmit \geq 0$.
% When $(f,g) = (\vub,\vlb)$, one no longer has $\dt \geq 0$ since $\Vubmit$ can be larger than
% $\Vlbt$.
% However, we can obtain a weaker bound of the form,
% \[
% \dt = 
% \Vlbt(\alloct) - \Vubmit(\allocmit)
% =  \max\Vubt - \max\Vubmit - 2\sum_i \sigmait(\sit)
% \geq - 2\sqrt{2}\sigma\betat  n K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}.
% \]
% % \[
% % \EE[\dt|\Et] \geq 
% % 
% % This leads to the following bounds for $\Gt(\alloct) - \Fmit(\allocmit)$.
% % \begin{align*}
% % \Gt(\alloct) - \Fmit(\allocmit) \geq 0  \hspace{0.15in}
% %     \text{if $(f,g) = (\vlb,\vub), (\vbar,\vbar)$},
% % \hspace{0.4in}
% % \EE[\Gt(\alloct) - \Fmit(\allocmit)|\Et] \geq 0  \hspace{0.15in}
% % \text{if $(f,g) = (\vub,\vlb)$}.
% % \end{align*}
% % 
% We can now bound the utilities for the various $f,g$ values as given in the theorem.
% We will first consider the cases $(f,g) = (\vlb,\vub)$ and $(f,g) = (\vbar,\vbar)$ when
% the agent is participating by bids.
% We have, $\utilit=\ct + \dt\geq 0$ a.s. for all $t\notin\Expl$.
% That is, the algorithm is instantaneously individually rational.
% If $(f,g)=(\vub, \vlb)$ then,
% $\UiT = \sum_t\utilit
% \geq - 3\sqrt{2}n\sigma \betat K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}$ a.s..
% 
% 
% If agent $i$ participates by rewards truthfully, by the three previous displays,
% we have,
% \begin{align*}
% \EE[\UiT] \geq
% \sum_{t\notin \Expl}\EE[\utilit] \geq
% \begin{cases}
% - 3\sqrt{2} \sigma\betat K^{\nicefrac{1}{3}} \Ttwth + 4, \;& \text{if }
%     (f,g) = (\vlb, \vub),
% \\
% - \frac{3}{\sqrt{2}} \sigma\betat K^{\nicefrac{1}{3}} \Ttwth + 4,
% \;& \text{if }
%     (f,g) = (\vbar, \vbar),
% \\
% - 3\sqrt{2} n \sigma\betat K^{\nicefrac{1}{3}} \Ttwth + 4, \;& \text{if }
%     (f,g) = (\vub, \vlb).
% \end{cases}
% \end{align*}
% % The claim follows by writing $\EE[\UiT] = \sum_t\EE[
% % 
% % $\EE[\utilit] = \EE[\ct + \dt] \geq 0$ for all $t\notin\Expl$.
% % That is, the algorithm is individually rational in expectation.
% % \vspace{-0.3in}
% \qedwhite

% \vspace{0.1in}
% \subsubsection{Truthfulness: Proof of Theorem~\ref{thm:eemain}.\ref{thm:eetruthful}}
% \label{sec:eetruthful}
% 
% Our main tool in the proof of truthfulness will be Lemma~\ref{lem:decomposition}.
% There, we will set $\pi_2$ to be the (non-truthful) policy $\pi$ in the theorem statement
% and $\pi_1$ to be a truthful policy played either via bids or rewards.
% $\pi^r_t$ is the policy which submits bids or rewards according
% to $\pi$ for time steps $1,\dots,r-1$.
% Therefore, the allocations for rounds $1,\dots,r$ will be based on these $\pi$ submissions.
% After experiencing the allocation for the $r$\ssth round, it will switch to a truthful policy,
% and the allocations for rounds $r+1$ onwards are based on these truthful submissions.
% %  then
% % switches to a truthful policy.
% % Precisely, the allocations are based on the values reported by $i$ according to $\pi$
% If participating by bids, this means it will change the bid function, and if participating by rewards,
% it means it will replace the reported rewards $\Yit$ from previous steps with the true
% rewards $\Xit$ and continue playing truthfully from round $r+1$ onwards.
% 
% 
% \emph{Proof.}
% By substituting the appropriate terms in Lemma~\ref{lem:decomposition}, we have
% \begin{align*}
% \label{eqn:utildecomposition}
% \numberthis
% \UpiiT - \UiT = \sum_{t=1}^T \utilipit - \utilitmot  + \sum_{t=2}^T \utilitmot - \utilit,
% \end{align*}
% where $\utilipit, \utilipptt{r}{t},\utilit$ are respectively the utilities
% of agent $i$ when following policies $\pi$, $\pi^r_t$ and truthful reporting.
% We will also denote the outcomes at time $t$ as $\allpit,\allpptt{r}{t},\alloct$ and
% the allocations for agent $i$ at time $t$ as $\sipit,\sipptt{r}{t},\sit$ for these
% policies respectively.
% As mentioned in Remark~\ref{rem:decomposition}, we will first
% fix any randomness 
% and simply look at the change in utility for agent $i$ when switching from $\pi$ to truthful
% reporting.
% 
% % Moreover, we will let 
% First, consider the second summation, where we claim that each term inside the summation is $0$.
% To see this, note that $\pi^{t-1}_t$ is also participating truthfully at round $t$.
% It has replaced its reported rewards with its true realised rewards in the previous rounds.
% The mechanism only uses rewards reported in the exploration rounds to decide allocations on
% the exploitation rounds, and the allocations in the exploration rounds are chosen independent
% of the bids/rewarks reported by the agent.
% As the allocation and prices in round $t$ will be the same for both policies,
% $\utilitmot = \utilit$.
% 
% Now turn to the first summation in the RHS of~\eqref{eqn:utildecomposition}.
% In the remainder of the proof,
% $\git$ will denote the appropriate quantity, either $\vlbit$, $\vbarit$, or $\vubit$ depending
% on the value of hyperparameter $g$,
% % in~\eqref{eqn:learnterms},~\eqref{eqn:bidterms}
% for agent $i$ when following $\pi^{t-1}_t$.
% Since, at time $t$, she has switched to being truthful, this is computed using her actual
% rewards.
% % This will be different from the corresponding quantity at time $t$ when following $\pi$ since the
% % values being used are not truthful.
% Similarly, let $\Gt$ denote either $\Vlbt$, $\Vbart$, or $\Vubt$
% for the welfare 
% % % $\Fmit$
% when agent $i$ follows  $\pi^{t-1}_t$.
% Using these, we can write for $t\notin\Expl$,
% % To make the dependence explicity, write the upper bound in~\eqref{eqn:eeterms} for agent $j$ when
% % agent $i$ follows $\pi^{t-1}_t$ as $\
% % we use Fact~\ref{fac:algoutils} to write,
% \begingroup
% \allowdisplaybreaks
% \begin{align*}
% \numberthis
% \label{eqn:eetruthcalcs}
% \utilipit - \utilitmot \;&=\; \bigg(\vali(\sipit) +
%                                 \Big(\valmech(\allpit) + \sum_{j\neq i}\gjt(\allpit) \Big) -
%                                 \max_\alloc\Fmit(\alloc) \bigg) \\
%             &\hspace{0.8in} -   \bigg(\vali(\sitmot) +
%                                 \Big(\valmech(\alltmot) + \sum_{j\neq i}\gjt(\alltmot) \Big) -
%                                 \max_\alloc\Fmit(\alloc) \bigg), \\
%     &=\;  \vali(\sipit) - \vali(\sitmot) + 
%                 \Big(\valmech(\allpit) + \sum_{j\neq i}\gjt(\allpit) \Big) -
%                 \Big(\valmech(\alltmot) + \sum_{j\neq i}\gjt(\alltmot) \Big), \\
%     &=\;  (\vali(\sipit) - \git(\sipit)) + (\git(\sitmot) - \vali(\sitmot)) \,+\, \\
%      &\hspace{0.8in}
%        \Big(\underbrace{\valmech(\allpit) + \sum_{i=1}^n\gjt(\allpit) }_{\Gt(\allpit)}\Big) -
%       \Big(\underbrace{\valmech(\alltmot) + \sum_{i=1}^n\gjt(\alltmot)}_{\Gt(\alltmot)} \Big),
%         \\
%     &\leq\;(\vali(\sipit) - \git(\sipit)) + (\git(\sitmot) - \vali(\sitmot)).
% \end{align*}
% \endgroup
% Here, the first step substitutes expressions for $\utilipit,\utilitmot$ from
% Fact~\ref{fac:vcgutils}.
% The $\max_\alloc\Fmit(\alloc)$ terms are cancelled out in the second step; 
% they will be the same for both policies $\pi, \pi^{t-1}_t$ since
% it is computed using the rewards reported by other agents in rounds $1,\dots,t-1$
% and hence does not depend on the fact that agent $i$ has switched policies in the current round.
% The third step adds and subtracts $\git(\sipit) + \git(\sitmot)$ and observes
% that the last two terms are $\Gt(\allpit), \Gt(\alltmot)$, where, recall
% % In the next step, we use the fact that $\Gt(a
% $\Gt$ is the appropriate quantity computed \emph{after}
% agent $i$ switches to truthful reporting.
% To obtain the last step,
% recall that $\alltmot = \argmax_\alloc \Vubt(\alloc)$ by line~\ref{lin:alloct} of
% Algorithm~\ref{alg:vcglearn}.
% As we observed in Section~\ref{sec:eerational},
% $\alltmot=\argmax_\alloc \Gt(\alloc)$ since $\Vlbt,\Vbart,\Vubt$ are vertically shifted functions
% and therefore, $\Gt(\alltmot) \geq \Gt(\allpit)$.
% % The last step uses the fact that $\alltmot =\argmax\Vubt$ as chosen by the mechanism
% % in Line~\eqref{eqn:lin:eealloct} of Algorithm~\ref{alg:vcgee} once agent $i$ has switched
% % 
% We emphasise that the above calculations do not use the fact that $\vubjt$ is an upper confidence
% bound on $\valj$ for an agent $j\neq i$; this may not be true since agent $j$ may not be truthful.
% Instead, it is simply treated as a function of rewards reported by agent $j$ in previous rounds.
% 
% To complete the proof, we can use the fact that that the $\git$ terms
% are computed under truthful reporting from agent $i$.
% % $\vubit$ is a truthful upper confidence bound.
% If the agent participates by bids, then $\git = \vali$ and hence
% $\utilipit - \utilitmot \leq 0$ a.s..
% Combining this with the fact that the utilities
% for all policies are the same during $t\in\Expl$, we have
% $\UpiiT - \UiT \leq 0$ a.s..
% For an agent participating by rewards,
% under $\Eit$,
% \begin{align*}
% \vali(\sipit) - \git(\sipit) + \git(\sitmot) - \vali(\sitmot)
% &= 
% \vali(\sipit) - \vubit(\sipit) + \vubit(\sitmot) - \vali(\sitmot)
% \\
% &\leq
% 2\betat\sigmait(\mapfuni(\allocmit)) \;\leq\;
%       2\sqrt{2}\betat \sigma K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}.
% \end{align*}
% Here, we have used the fact
% % regardless of the value of $g$,
%  the widths of the confidence intervals are all equal.
% % Moreover, $\EE[\vbarit(s)] = \vali(s)$ for all $s$ since $\Nit(s) = \qt$ deterministically.
% This leads us to $\EE[\utilipit - \utilitmot|\Eit] \leq 2\sqrt{2}\betat \sigma
% K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}$
% and consequently,
% \[
% \EE[\UpiiT - \UiT] = \sum_{t} \EE[\utilipit - \utilitmot|\Eit] + \sum_t\PP(\Eit)
% \leq 3\sqrt{2}\betaT K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}} + 4.
% % \vspace{-0.5in}
% \]
% \qedwhite


% In our analysis of \vcgucb, we will find that 



==> prelims_app.tex <==


% \vspace{0.2in}

% Next, we present the proofs of our theoretical results in
% Sections~\ref{sec:prelims_app}-\ref{sec:vcglearnanalysis}.
% In Section~\ref{sec:prelims_app}, we state some notation and prove some preliminary results.
% Section~\ref{sec:lb_app} proves the lower bound in Theorem~\ref{thm:lowerbound}
% while Section~\ref{sec:vcglearnanalysis} proves the results in Theorems~\ref{thm:eemain}
% and~\ref{thm:ucbmain}.

% \section{Some Useful Results}
\section{Notation \& Some Preliminary Results}
\label{sec:prelims_app}
% 
% 
% \subsection{Setup and Notation}
\label{sec:setup_app}

% We will begin with some results
% that will be useful throughout our analysis.pre

In this section, we first state some notation and definitions that will be used throughout
our proofs in Sections~\ref{sec:setup_app}--\ref{sec:}.
We will then prove some  results that will be useful throughout our analysis.
$\EE, \PP$ will denote expectations and probabilities.
$\EEt, \PPt$ will denote expectation and probability when conditioned on observations
up to time $t-1$; for example, $\PPt(\cdot) = \PP(\cdot|D_t)$, where
$D_t = \{\sil, \Yil\}_{i\leq n, \ell\leq t-1}$.

Recall that $\allocopt = \argmax_\alloc \Val(\alloc)$ is the socially optimal outcome.
Let $\siopt = \mapfuni(\allocopt)$ be the allocation for agent $i$ at the optimum.
Similarly, $\Valmi$ and $\allocmiopt$, defined below, will denote the welfare without
agent $i$ and its optimiser respectively.
\begin{align*}
\Valmi(\alloc) = \valmech(\alloc) + \sum_{j\neq i} \vali(\alloct),
\hspace{0.35in}
\allocmiopt = \argmax_{\alloc\in\Alloc}\Valmi(\alloc).
\numberthis
\label{eqn:Valmidefn}
\end{align*}


Our first result is a straightforward fact regarding agent and seller utilities in the
VCG mechanism.

\insertprethmspacing
\begin{fact}
\label{fac:vcgutils}
When allocations and prices are chosen according to the VCG mechanism,
\begin{align*}
\utiliopt &= \vali(\siopt) - \priceiopt = \Val(\allocopt) - \Valmi(\allocmiopt),
\\
\utilmechopt &= \valmech(\allocopt) + \sum_{i=1}^n\priceiopt =
            \sum_{i=1}^n\Valmi(\allocmiopt) - (n-1)\Val(\allocopt).
\end{align*}
\end{fact}


% For our second result, we will rewrite the expressions for
% the regret terms~\ref{eqn:regret} in a way that is convenient to analyse.
Our second result expresses the regret terms in a way that is convenient for analysis.
Define:
\begin{align*}
\numberthis
\label{eqn:HTWTdefn}
\HT = \frac{1}{T}\sum_{i=1}^n\sum_{t=1}^T\left(\priceit + \Valmi(\alloct)\right),
\hspace{0.5in}
\WT =  \HT - \sum_{i=1}^n \Valmi(\allocmiopt).
\end{align*}
% Here, $\Valmi$ is defined in~\eqref{eqn:welfaredefns}.
$\HT$ is computed using observations from rounds $1$ to $T$, and can be thought of as
the algorithm's estimate of $\sum_i \Valmi(\allocopt)$ at the end of $T$ rounds.
The following lemma expresses $\RaT$ and $\RmechT$ in terms of $\RT$ and $\WT$.

\insertprethmspacing
\begin{lemma}
\label{lem:WTdecomposition}
Let $\RaT, \RmechT, \RT$ be as defined in~\eqref{eqn:regret}.
Then,
\[
\RaT = n\RT + T\WT,
\hspace{1in}
\RmechT = -(n-1)\RT - T\WT.
\]
\end{lemma}
\begin{proof}
% Recall from Fact~\ref{fac:vcgutils},
% $\utiliopt &= \vali(\siopt) - \priceiopt = \Val(\allocopt) - \Valmi(\allocmiopt)$, and
% $\utilmechopt = \valmech(\allocopt) + \sum_{i=1}^n\priceiopt =
%             \sum_{i=1}^n\Valmi(\allocmiopt) - (n-1)\Val(\allocopt)
Let $\hit=\priceit + \Valmi(\alloct)$ so that
$\HT =\frac{1}{T}\sum_{i=1}^n\sum_{t=1}^T \hit$.
For agent $i$, we can use Fact~\ref{fac:vcgutils} and the fact that
$\utilit = \vali(\alloct) - \priceit = \Val(\alloct) - \hit$ to obtain,
\[
\utiliopt - \utilit =  (\Val(\allocopt) - \Val(\allocmiopt)) - (\Val(\alloct) - \hit)
    = (\Val(\allocopt) - \Val(\alloct)) + (\hit - \Val(\allocmiopt)).
\]
Then, since $\RaT = \sum_i\sum_t (\utiliopt - \utilit)$, we have
\begin{align*}
\RaT &= \sum_{t=1}^T \sum_{i=1}^n 
\left((\Val(\allocopt) - \Val(\alloct)) + (\hit - \Val(\allocmiopt))\right)
\\
&= n \sum_{t=1}^T (\Val(\allocopt) - \Val(\alloct)) \;+\;
        T\left(\HT - \sum_{i=1}^n\Valmi(\allocmiopt)\right) \,.
\end{align*}
This proves the first claim.
For the seller, at time $t$, we observe
\begin{align*}
\utilmecht = \valmech(\alloct) + \sum_{i=1}^n\priceit 
    = \valmech(\alloct) + \sum_{i=1}^n \hit - \sum_{i=1}^n \Valmi(\alloct)
    = \sum_{i=1}^n \hit - (n-1)\Val(\alloct).
\end{align*}
As before, we can now use Fact~\ref{fac:vcgutils} to write,
\begin{align*}
\RmechT &= \sum_{t=1}^T\left(\utilmechopt - \utilmecht\right)
    = \sum_{t=1}^T\sum_{i=1}^n \left(\Valmi(\allocmiopt) - \hit\right)
    + (n-1) \sum_{t=1}^T(\Val(\alloct) - \Val(\allocopt)).
%     = \sum_{t=1}^T\sum_{i=1}^n \left(\Valmi(\allocopt) - \hit\right)
%     + (n-1) (\Val(\alloct) - \Val(\alloct)).
% \\
%     &= T\left(\sum_{i=1}^n\Valmi(\allocmiopt) - \HT\right)
%     - (n-1)\RT.
\end{align*}
The claim follows by observing that the first term in the RHS is $-T\WT$ and that the second term
is $-\RT$.
\end{proof}

Our next result helps us quantify the difference when an agent submits her realised
rewards truthfully vs when she does not.
To state this lemma,
consider a general setting where an agent interacts with a stateful environment over $T$ rounds.
That is, on each round $t$, she takes some action $a_t$, collects an observation $y_t$,
and receives a reward $z_t$ (possibly unobserved).
The actions taken by this agent can affect the state of the environment, and, in turn, the
observations and rewards depend on this state.
The agent may use the observations to inform decisions in future rounds.
Generally speaking, the agent is following a policy $\pi$ to make her decisions, which maps
past actions and observations to an action for the current time step.
Let $\zpit$ be the reward at time $t$ when following such a policy $\pi$ from round 1.
Let $\ZpiT = \sum_{t=1}^T\zpit$ denote the sum of rewards.
The following lemma will help us quantify the difference between two policies.
% The following lemma will help us quantify the difference of two policies $\pi_1, \pi_2$ in the
% above scenario.

\insertprethmspacing
\begin{lemma}
\label{lem:decomposition}
Let $\pi_1, \pi_2$ be two different policies in the above set up and $\ZpoT, \ZptT$ be the sum
of rewards.
Let $\pi^r_t$ denote the policy which follows $\pi_2$ for rounds $1,\dots,r$ and then
follows $\pi_1$ for rounds $r+1,\dots,T$.
Let $\zpptt{r}{t}$ denote the reward at time $t$ when following policy $\pi^r_t$.
Then,
\begin{align}
\label{eqn:decomposition}
\ZptT - \ZpoT \;\;= \sum_{t=1}^T (\zptt - \ztmot) \;+\;\sum_{t=2}^T (\ztmot - \zpot).
\end{align}
\begin{proof}
The claim follows by adding and subtracting $\sum_{t=1}^T \ztmot$, rearranging the terms,
and noting that $\zpptt{0}{1} = \zpptt{\pi_1}{1}$.
\end{proof}
\end{lemma}
\insertpostthmspacing
To see how we will use Lemma~\ref{lem:decomposition} in our truthfulness proofs,
let $\pi_1$ denote the truthful submission of bids or rewards and let
$\pi_2$ be any other (non-truthful) policy.
Then $\pi^r_t$ is the policy which follows $\pi_2$ for rounds $1,\dots,r$ and then switches to
truthful submission for the remaining rounds.
The terms inside the first summation in~\eqref{eqn:decomposition} denote the instantaneous
difference in being truthful, which can be controlled using proof techniques
similar to that of truthfulness in the VCG mechanism.
However, an agent may choose to be strategic over multiple rounds, say
by achieving only small rewards in early rounds, with the intent of gaining in the long term.
This is reflected in the second summation, and we will use properties of our algorithm,
along with the fact that the agent is currently being truthful,
to control this term.
% In the design of our algorithm,
% Lemma~\ref{lem:decomposition} was instructive in characterising the properties necessary
%  to achieve truthfulness.
% In particular, we will use the fact that for each term in the second summation, both policies
% are behaving truthfully at the current time step.

\insertprethmspacing
\begin{remark}
\label{rem:decomposition}
\emph{
When the observations $y_t$ are stochastic and/or there is randomness in the
policies $\pi_1,\pi_2$, Lemma~\ref{lem:decomposition} holds in an almost sure sense.
To see this, say that observations for all time steps, actions
and states of the environment are generated according to some source of randomness $\eta_o$.
The agent only sees observations according to the current state and its current action.
Second, policy $\pi_i$ may choose its action as a function of past observations and some
external source of randomness $\eta_{i}$.
% precisely, the distribution it samples its actions from at time $t$ is measurable with
% respect to past actions and observations $\{(a_s, y_s)\}_{s<t}$.
Then,~\eqref{eqn:decomposition} holds when you fix $\eta_o, \eta_{1}$, and $\eta_{2}$.
% TODO: maybe don't need to emphasise this as much?
}
\end{remark}


Finally, we will repeatedly use the following two results in our proofs.

\insertprethmspacing
\begin{lemma}
\label{lem:boundmax}
Let $f_1, f_2:\Xcal\rightarrow\RR$ for some finite set $\Xcal$ such that $f_1(x)-f_2(x)\leq\epsilon$
for all $x\in\Xcal$ and a given $\epsilon\geq 0$.
Then $\max f_1 - \max f_2 \leq \epsilon$.
\begin{proof}
Let $x_i=\argmax f_i$. Then, $f_1(x_1) - f_2(x_2) \leq f_2(x_1) - f_2(x_2) + \epsilon \leq \epsilon$.
% The other side follows similarly.
\end{proof}
\end{lemma}


\insertprethmspacing
\begin{lemma}
\label{lem:subounds}
\;$\sum_{t=1}^n t^{-\nicefrac{1}{2}} \leq 2n^{\nicefrac{1}{2}}$,
\quad $\sum_{t=1}^n t^{-\nicefrac{1}{3}} \leq \frac{3}{2}n^{\nicefrac{2}{3}}$.
\begin{proof}
By bounding the summation of a decreasing function by an integral we have for $r\in[0, 1]$,
$\sum_{t=1}^n t^{-r} \leq 1 + \int_1^n t^{-r}\ud t \leq 1 + \frac{n^{1-r}}{1-r} -\frac{1}{1-r}
\leq  \frac{n^{1-r}}{1-r}$.
Setting $r=1/2, 1/3$ yields the results.
\end{proof}
\end{lemma}



==> ucb_app.tex <==


\vspace{0.1in}
\subsection{Proof of Theorem~\ref{thm:ucbmain}}
\label{sec:ucb_app}

% In this section, we analyse Algorithm~\ref{alg:vcglearn} when $\estmethod=\estopt$.


% where Appendix~\ref{sec:eewelfare} bounds the welfare regret to establish the first part of the
% theorem.
% \ref{sec:eeagentregret} bounds the agent regret,
% \ref{sec:eesellerregret} bounds the seller regret,
% and~\ref{sec:eeagentseller} proves the second part of the theorem.
% Sections~\ref{sec:eerational} and~\ref{sec:eetruthful} establish individual rationality and
% truthfulness to prove the last two statements of the theorem.
% % We first state a complete version of the theorem which includes all constants.
% Recall that in the first two results, we assume
% that all agents are truthful, while in the last two, we do not.


% \vspace{0.1in}
% \subsubsection{Bounding the Welfare Regret: Proof of Theorem~\ref{thm:ucbmain}.\ref{thm:ucbwelfare}}
% \label{sec:ucbwelfare}
% 
% \emph{Proof.}
% We use Lemma~\ref{lem:RTgenbound} to bound the welfare regret.
% By Lemma~\ref{lem:Etcbound}, we have $\sum_t\PPt(\Etc) \leq 6n$.
% % To bound the second term in the RHS of Lemma~\ref{lem:RTgenbound},
% The following argument will help us bound $\sum_{t\notin\Expl}\sigmait(\sit)$ for each agent
% $i$:
% % we use the following argument which is commonl
% \begin{align*}
% \label{eqn:sqrtSTbound}
% \numberthis
% % \sum_{t\notin\Expl} \betat \sigmait(\sit) \leq
% % \betaT\sigma \sum_{t\notin\Expl} \frac{1}{\sqrt{\Nit(\sit)}} \leq
% % \betaT\sigma \sum_{t\notin\Expl} \frac{1}{\sqrt{\Nit(\sit)}} \leq
% \sum_{t\notin\Expl} \frac{1}{\sqrt{\Nit(\sit)}} 
% &\leq
% \sum_{t>K} \frac{1}{\sqrt{\Nit(\sit)}} \leq
% % \sum_{t\notin\Expl} \frac{1}{\sqrt{\Npit(\sit)}} =
% \sum_{s\in\Scal}  \sum_{j=1}^{\NiT(s)} \frac{1}{\sqrt{j}}
% \\
% &\leq 2 \sum_{s\in\Scal} \sqrt{\NiT(s)}
% \leq 2 \sqrt{|\Scal|(T-qK)}
% \leq 2 \sqrt{|\Scal|T}.
% \end{align*}
% The first step simply adds more terms to the summation.
% The second step observes that the summation can be written as $|\Scal|$ different summations,
% one for each $s\in\Scal$.
% % that this summation is smaller than if we had summed
% The third step uses Lemma~\ref{lem:subounds}.
% These results along with Lemma~\ref{lem:Etcbound} yield:
% \begin{align*}
% \EE[\RT] \leq 6 \Vmax n + 4\sigma n \betaT \sqrtST + 3\KotTtt.
% \numberthis
% \label{eqn:ucbwelfareregbound}
% \end{align*}
% The claim follows by substituting for $\betaT$.
% \qedwhite

% \vspace{0.05in}
% \subsubsection{Bounding the Agent Regret}
% \label{sec:ucbagentregret}
% 
% We will use Lemma~\ref{lem:RiTgenbound} and bound the $\at, \bt$ terms for the
% different choices of hyperparameters $f, g$.
% First, $\at$ is bounded identically to obtain the upper bound in~\eqref{eqn:atagent};
% this uses the fact that even when $\estmethod=\estopt$, there will have been $\qT$ exploration
% phases by round $T$.
% However,
% we will obtain tighter bounds for $\bt$.
% 
% 
% When $g=\vub$, $\git=\vubit$ and $\Gmit=\Vubmit$.
% We therefore have,
% $\bt = \vubit(\sit) - \vlbit(\sit) = 2\betat\sigmait(\sit)$ if the agent is participating
% by rewards and $\bt=0$ if she is participating by bids.
% Similarly, when $g=\vlb$, 
% $\bt= \Vubt(\alloct) - \Vlbt(\alloct) = 2 \betat\sum_i\sigmait(\alloct)$,
% and when $g=\vbar$,
% $\bt= \vbarit(\sit) - \vlbit(\sit) + \Vubt(\alloct) - \Vbart(\alloct)
% = \betat\sigmait(\sit) + \betat\sum_i\sigmait(\alloct)$.
% Using a similar argument to~\eqref{eqn:sqrtSTbound},
% we obtain the following bounds on the sum of $\bt$'s when $t\notin\Expl$:
% \begin{align*}
% \numberthis
% \label{eqn:btagentopt}
% \sum_{t\notin\Expl} \EE[\bt|\Et] \,\leq\;
%     \begin{cases}
%         \;4\betaT \sigma n \sqrtST
%             \hspace{0.2in}&\text{if $g=\vlb$}, \\
%         \;2\betaT \sigma (n + \kappaiv) \sqrtST
%             \hspace{0.2in}&\text{if $g=\vbar$}, \\
%         \;4 \kappaiv \betaT \sigma \sqrtST
%             \hspace{0.2in}&\text{if $g=\vub$}.
%     \end{cases}
% \end{align*}
% Recall that $\kappaiv=1$ if the agent is participating by rewards, and $\kappaiv=0$ if she is
% participating by bids.
% We will combine this result with~\eqref{eqn:RiTbound} and~\eqref{eqn:atagent} to bound the
% agent regret for different $f,g$ hyperparameter choices in Section~\ref{sec:ucbagentseller}.




% \vspace{0.05in}
% \subsubsection{Bounding the Seller Regret}
% \label{sec:ucbmechregret}
% \label{sec:ucbsellerregret}
% 
% Following along the same lines as Section~\ref{sec:eemechregret}, we will use
% Lemma~\ref{lem:RmechTgenbound} to control the seller regret, and moreover,
% use the expression in~\eqref{eqn:Atmech} to bound the $\EE[\Amit|\Et]$ terms.
% The same bounding technique can be used since, even when $\estmethod=\estopt$,
%  there will have been $\qT$ exploration phases by round $T$.
% 
% To bound the $\Bt$ terms, we first observe that under $\Et$, $\Val(\allocopt) \geq \Val(\alloct)
% \geq \Vlbt(\alloct)$.
% When $g=\vlb$, we have $\Gt=\Vlbt$, and therefore $\Bt \leq 0$.
% When $g=\vub$, we have $\Gt=\Vubt$, and therefore  $\Bt \leq \Vubt(\alloct) - \Vlbt(\alloct) =
% 2\betat\sum_i\sigmait(\sit)$.
% And when $g=\vbar$, $\Bt \leq  \betat\sum_i\sigmait(\sit)$.
% Putting these results together and using a similar argument to~\eqref{eqn:sqrtSTbound},
% we obtain the following bounds on the sum of $\Bt$'s:
% \begin{align*}
% \label{eqn:Btmechopt}
% \numberthis
% (n-1)\sum_{t\notin\Expl} \EE[\Bt|\Et] \espleq
%     \begin{cases}
%         \;0 &\text{if $g=\vlb$}, \\
%         \;2\sigma\betaT n(n-1) \sqrtST
%         \hspace{0.2in} &\text{if $g=\vbar$}, \\
%         \;4\sigma\betaT n(n-1) \sqrtST
%         \hspace{0.2in} &\text{if $g=\vub$}.
%     \end{cases}
% \end{align*}
% 
% 
% % \vspace{0.1in}
% \subsubsection{Proof of Theorem~\ref{thm:ucbmain}.\ref{thm:ucbagentseller}}
% \label{sec:ucbagentseller}
% 
% 
% \emph{Proof.}
% The claims follow by combining the bounds in~\eqref{eqn:atagent},~\eqref{eqn:btagentopt},
% and Lemma~\ref{lem:RiTgenbound} for the agent and the bounds
% in~\eqref{eqn:Atmech},~\eqref{eqn:Btmechopt}, and Lemma~\ref{lem:RmechTgenbound} for the seller.
% % 
% % The claims simply follow by combining the bounds in~\eqref{eqn:RiTbound},~\eqref{eqn:atagent},
% % and~\eqref{eqn:btagentopt} for the agent and the bounds
% % in~\eqref{eqn:RmechTbound},~\eqref{eqn:Atmech}, and~\eqref{eqn:Btmechopt} for the seller.
% % Let $\kappaiv=1$ when the agent participates by rewards and $\kappaiv = 0$ when she participates
% % by bids.
% % Also observe that $3\sqrt{2}\betaT \leq 10\sqrt{\logST}$.
% When $(f,g) = (\vlb,\vub)$,
% \begin{align*}
%  \EE[\RiT] &\leq
%        6n  + 4\sigma\betaT\kappaiv\sqrtST + 3\valiexpl K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}, \\
%  \EE[\RmechT] &\leq
%        6n\Vmax + 4\sigma\betaT n(n-1) \sqrtST + \Big(3\Vmax  + 3\sqrt{2}\sigma \betaT n(n-1) \Big) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}.
% \end{align*}
% When $(f,g) = (\vlb,\vlb)$,
% \begin{align*}
%  \EE[\RiT] &\leq
%        6n + 4\sigma\betaT n\sqrtST +  3\valiexpl K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}, \\
%  \EE[\RmechT] &\leq
%        6n\Vmax + \Big(3\Vmax  + 3\sqrt{2}\sigma \betaT n(n-1) \Big) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}.
% \end{align*}
% When $(f,g) = (\vub,\vub)$,
% \begin{align*}
%  \EE[\RiT] &\leq
%        6n + 4\sigma\betaT\kappaiv\sqrtST + (3\valiexpl + 3\sqrt{2}\sigma\betaT n)K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}, \\
%  \EE[\RmechT] &\leq
%        6n\Vmax + 4\sigma\betaT n (n-1) \sqrtST + 3\Vmax K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}.
% \end{align*}
% When $(f,g) = (\vub,\vlb)$,
% \begin{align*}
%  \EE[\RiT] &\leq
%        6n + 4\sigma\betaT n \sqrtST + (3\valiexpl + 3\sqrt{2}\sigma\betaT n)K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}, \\
%  \EE[\RmechT] &\leq
%        6n\Vmax + 3\Vmax K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}.
% \end{align*}
% 
% \vspace{-0.2in}
% \qedwhite

% \subsubsection{Proof of Theorem~\ref{thm:ucbmain}.\ref{thm:ucbmaxregret}}
% \label{sec:ucbmaxregret}
% 
% \emph{Proof.}
% We will use Lemma~\ref{lem:MaxRegretgenbound} to bound the maximum of the three regret quantities.
% Since there will have been $\qT$ exploration phases in $T$ rounds, we use the expression
% in~\eqref{eqn:Amitmodbound} to bound the sum of $\EE[|\Amit||\Et]$ terms.
% % The same bounding technique can be used since, even when $\estmethod=\estopt$,
% % By repeating the argument in Section~\ref{sec:eemaxregret}, we can obtain
% % $|\Amit| \leq 2\sqrt{2}\sigma\betat (n-1)\Kottmot$.
% % 
% Next, let us turn to the $|\Bt|$ terms in the RHS of
% Lemma~\ref{lem:MaxRegretgenbound}.
% % our argument will follow along similar lines to Section~\ref{sec:ucbsellerregret}.
% % where we have already obtained bounds for $\Bt$.
% When $g=\vlb$, we already saw in Section~\ref{sec:ucbsellerregret} that $\Bt \leq 0$.
% Moreover, $-\Bt = \Val(\allocopt) - \Vlbt(\alloct) \leq \Vubt(\alloct) - \Vlbt(\alloct)
% \leq 2\betat\sum_i\sigmait(\sit)$.
% Similarly, when $g=\vub$, we already saw $\Bt \leq 2\betat\sum_i\sigmait(\sit)$.
% Moreover, $-\Bt = \Val(\allocopt) - \Vubt(\alloct) \leq 0$.
% Finally, when $g=\vbar$,
% both $\Bt, -\Bt$ can be bounded by $\betat\sum_i\sigmait(\sit)$.
% In all cases, we have $|\Bt| \leq 2\betat\sum_i\sigmait(\sit)$ and therefore,
% by following the same calculations in~\eqref{eqn:sqrtSTbound},
% we have,
% \[
% (n-1)\sum_{t\notin\Expl} \EE[|\Bt|\,|\Et] \leq 4\sigma\betaT n(n-1)\sqrtST.
% \]
% % This leads us to the following bound on $\EE[|\RmechT|]$,
% % \[
% % \EE[|\RmechT|] \leq
% %        6n\Vmax + 4\sigma\betaT n(n-1) \sqrtST + \Big(3\Vmax  +
% %         3\sqrt{2}\sigma \betaT n(n-1) \Big) K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}}.
% % \]
% % The result follows by combining the above with~\eqref{eqn:maxregbound}
% % and~\eqref{eqn:RmechTabsbound}.
% The claim follows by combining the above with Lemma~\ref{lem:MaxRegretgenbound},
% the bound on the welfare regret in~\eqref{eqn:ucbwelfareregbound},
% and Lemma~\ref{lem:Etcbound} to control $\sum_{t\notin\Expl}\PPt(\Etc)$.
% \qedwhite


% \vspace{0.1in}
% \subsubsection{Individual Rationality: Proof of Theorem~\ref{thm:ucbmain}.\ref{thm:ucbrational}}
% \label{sec:ucbrational}
% 
% \emph{Proof.}
% For all agents, $\utilit\geq 0$ when $t\in\Expl$, so let us consider $t\notin\Expl$.
% As in Section~\ref{sec:eerational},
% we write $\utilit = \ct + \dt$ where $\ct,\dt$ are as defined in~\eqref{eqn:utilitirdecomp}.
% % we write using Fact~\ref{fac:algoutils},
% % \[
% % \utilit = \underbrace{\vali(\sit) - \git(\sit)}_{\ct} + \underbrace{\Gt(\alloct) -
% % \Fmit(\allocmit)}_{\dt}.
% % \]
% First consider $\ct$.
% If agent $i$ participates by bids truthfully, $\git = \vali$ and hence $\ct=0$.
% To bound $\ct$ when she participates by rewards truthfully, 
% let $\ctildet = \max(0, \git(\sit) - \vali(\sit))\geq 0$.
% Clearly, $\ct \geq -\ctildet$.
% % Now, conditioning on $\Eit$~\eqref{eqn:Eitdefn}, we have
% Observing that  $\vali\leq \vubit$ under $\Eit$~\eqref{eqn:Etdefn}, we have,
% \[
% \EE[\ctildet|\Eit] \leq 0 \hspace{0.10in}\text{if $g=\vlb$},
% % \hspace{0.3in}
% % \EE[\ctildet|\Eit] \leq \betat \sigmait(\sit)
% %     \hspace{0.05in}\text{if $g=\vbar$},
% \hspace{0.5in}
% \EE[\ctildet|\Eit] \leq 2 \betat \sigmait(\sit)
%     \hspace{0.10in}\text{if $g=\vub$}.
% \]
% To bound $\dt$, first note that $\Vubt(\alloct) - \max\Vubmit \geq 0$ since
% $\Vubt = \Vubmit + \vubit$ and $\vubit \geq 0$.
% Therefore, when $g=\vub$,
% \begin{align*}
% &\dt = \Vubt(\alloct) - \Fmit(\allocmit) \geq \Vubt(\alloct) - \max\Vubmit \geq 0,
% \end{align*}
% and when $g=\vlb$,
% \begin{align*}
% \dt = \Vlbt(\alloct) - \Fmit(\allocmit) \geq \Vubt(\alloct) - \max\Vubmit -
% 2\betat\sum_j\sigmajt(\sjt) \geq - 2\betat\sum_j\sigmajt(\sjt).
% \end{align*}
% % \begin{align*}
% % \text{When $g=\vub$,} \hspace{0.4in}
% % &\dt = \Vubt(\alloct) - \Fmit(\allocmit) \geq \Vubt(\alloct) - \max\Vubmit \geq 0. \\
% % \text{When $g=\vlb$,} \hspace{0.4in}
% % &\dt = \Vlbt(\alloct) - \Fmit(\allocmit) \geq \Vubt(\alloct) - \max\Vubmit -
% % 2\betat\sum_j\sigmajt(\sjt) \geq - 2\betat\sum_j\sigmajt(\sjt).
% % \end{align*}
% Moreover, by following the same calculations as in~\eqref{eqn:sqrtSTbound}, we have
% $\sum_t \betat\sigmajt(\sjt) \leq 2\betaT \sqrtST$ for all agents $j$.
% Therefore, for an agent participating by bids,
% $\UiT \geq -4\betaT n \sqrtST$ if $g=\vlb$, and
% $\UiT \geq 0$ if $g=\vub$.
% % \begin{align*}
% % \UiT &\geq - \sum_{t\notin\Expl} \ct - \sum_{t\notin\Expl} \dt 
% % \geq \begin{cases}
% % -4\betaT n \sqrtST \hspace{0.8in} &\text{if $g=\vlb$}, \\
% % 0  \hspace{0.8in} &\text{if $g=\vub$}.
% % \end{cases}
% % \end{align*}
% For an agent participating by rewards,
% \begin{align*}
% \EE[\UiT] &\geq - \sum_{t\notin\Expl} \EE[\ctildet|\Eit]  - \sum_{t\notin\Expl} \PP(\Eitc)
%     + \sum_{t\notin\Expl} \EE[\dt]
% \geq \begin{cases}
% -4\betaT n \sqrtST  \,- 6 \hspace{0.8in} &\text{if $g=\vlb$}, \\
% -4\betaT \sqrtST  \,- 6\hspace{0.8in} &\text{if $g=\vub$}.
% \end{cases}
% % \geq - 3\sqrt{2}\kappa_g\sigma \betat K^{\nicefrac{1}{3}} T^{\nicefrac{2}{3}} - 6.
% \end{align*}
% % Here $\kappaiv=1$ if the agent participates by realised values and $\kappaiv=0$ otherwise.
% We emphasise that we have only assumed truthfulness from agent $i$, specifically
% in bounding $\ct$.
% To bound $\dt$, we have simply used a relation between $\Vubt$ and $\Vlbt$ which holds
% almost surely regardless of the rewards reported by other agents.
% \qedwhite

\vspace{0.1in}
\subsubsection{Truthfulness: Proof of Theorem~\ref{thm:ucbmain}.\ref{thm:ucbtruthful}}
\label{sec:ucbtruthful}

\emph{Proof.}
As we did for $\estmethod=\estee$, we will use Lemma~\ref{lem:decomposition} and
set $\pi_1, \pi_2, \pi^r_t$ as described in the beginning of Section~\ref{sec:eetruthful}.
This leads us to the expression in~\eqref{eqn:utildecomposition} for $\UpiiT-\UiT$.
The main difference is that now the mechanism uses all of the rewards reported by the agents,
and this needs to be accounted for when bounding the two summations.
%
In this proof, we will annotate quantities related to policy $\pi^{t-1}_t$ at time $t$ with a prime.
For example, $\vpubit:\Scal\rightarrow\RR$ (see~\eqref{eqn:learnterms})
will be the upper confidence bounds at time $t$ for agent $i$ when following $\pi^{t-1}_t$.
On the same note, $\Epit$ denotes the event that agent $i$'s true values fall within
the confidence interval at time $t$ when she follows $\pi^{t-1}_t$.

For the terms in the first summation in~\eqref{eqn:utildecomposition},
by repeating the calculations in~\eqref{eqn:eetruthcalcs}, we obtain
(using our above notation),
\begin{align*}
\utilipit - \utilitmot = (\vali(\sipit) - \gpit(\sipit)) + (\gpit(\sitmot) - \vali(\sitmot)) +
                            \Gpt(\allpit) - \Gpt(\alltmot).
\end{align*}
Recall that $(\gpit, \Gpt)$ denote
either $(\vplbit, \Vplbt)$, $(\vpbarit, \Vpbart)$ or $(\vpubit, \Vpubt)$ as per the value of
$g$ being $\vlb$, $\vbar$, or $\vub$.
% hyperparameter $g$---%
% when the agent is following policy $\pi^{t-1}_t$.
They are computed under truthful reporting from agent $i$.
If the agent participates by bids, then $\gpit = \vali$ and hence $\vali(s) - \gpit(s) = 0$ for all
$s$.
If she participates by rewards, then for all choices of $g\in\{\vlb,\vbar,\vub\}$,
\begin{align*}
\label{eqn:gdiffreasoning}
\numberthis
\EE[(\vali(\sipit) - \gpit(\sipit)) + (\gpit(\sitmot) - \vali(\sitmot)|\Epit] \leq
    2\sqrt{2}\sigma \betat K^{\nicefrac{1}{3}} t^{\nicefrac{-1}{3}}.
\end{align*}
This follows from the observation that when $g=\vub$,
the first term is less than $0$ while the second is less than
$2\betat\sigmait(\sitmot) \leq 2\sqrt{2} \sigma\betat \Kottmot$ by Lemma~\ref{lem:qTbound}
and the fact that there have been $\qt$ exploration phases;
a similar argument holds for $g=\vlb$, but with the terms reversed;
when $g=\vbar$, both terms are less than $\sqrt{2} \sigma\betat \Kottmot$.

Next, we use $\alltmot=\argmax_\alloc\Vpubt(\alloc)$
to bound the difference $\Gpt(\allpit) - \Gpt(\alltmot)$.
When $g=\vub$,
\begin{align*}
% \text{When $g=\vub$,} \hspace{0.2in}
&\Gpt(\allpit) - \Gpt(\alltmot) = \Vpubt(\allpit) - \Vpubt(\alltmot) \leq  0.
% \text{When $g=\vlb$,} \hspace{0.2in}
% &\Gt(\allpit) - \Gt(\alltmot) = \Vlbt(\allpit) - \Vlbt(\alltmot) \leq 
% \Vubt(\allpit) - \Vubt(\alltmot) + 2\betat\sum_i(\sigmait(\alltmot) - \sigmait(\allpit))
\end{align*}
When $g=\vlb$, we can use the fact that at round $t\notin\Expl$
all allocations will have been experienced by each agent at least $\qt$ times~\eqref{eqn:qtdefn} to obtain,
\begin{align*}
\Gpt(\allpit) - \Gpt(\alltmot) &= \Vplbt(\allpit) - \Vplbt(\alltmot) \\
&\leq 
\Vpubt(\allpit) - \Vpubt(\alltmot) + 2\betat\sum_i(\sigmapit(\sitmot) - \sigmapit(\allpit)) \\
&\leq 2\betat\sum_i\sigmapit(\alltmot)
 \leq 2\sigma \betat\sum_i \frac{1}{\sqrt{\qt}}
\leq 2\sqrt{2}\sigma \betat n \Kottmot.
\end{align*}
The last step uses Lemma~\ref{lem:qTbound}.
By a similar argument, we get
$\Gpt(\allpit) - \Gpt(\alltmot) \leq
\sqrt{2}\sigma \betat n \Kottmot$ when $g=\vbar$.
Now summing over all $t$ and using Lemma~\ref{lem:subounds}, we obtain
\begin{align*}
\label{eqn:optfirstbound}
\numberthis
\sum_{t\notin\Expl} \EE[\utilipit - \utilitmot | \Epit]
\leq
\begin{cases}
3\sqrt{2}\sigma (n + \kappaiv) \betaT \KotTtt  \hspace{0.2in}&\text{if $g=\vlb$}, \\
3\sqrt{2}\sigma (n/2 + \kappaiv) \betaT \KotTtt  \hspace{0.2in}&\text{if $g=\vbar$}, \\
3\sqrt{2}\sigma \kappaiv \betaT \KotTtt \hspace{0.2in}&\text{if $g=\vub$}.
\end{cases}
\end{align*}

We now move to the second summation in~\eqref{eqn:utildecomposition}.
To bound this term, we will use the fact that 
all agents except $i$ are adopting stationary policies.
Therefore
the rewards reported by any agent $j\neq i$ for any $s\in\Scal$ concentrates around some mean,
and we can apply Lemma~\ref{lem:Eitcbound} for that agent.
For the remainder of this proof,
$\valj(s)$ will denote the mean of this distribution.
This may not be equal to the true value of agent $j$ for outcome $s$ since she may not be
truthful.
$\Et,\Ept$ denote the events that $\valj(s)$ falls within
the confidence intervals $(\vlbjt(s),\vubjt(s))$, $(\vplbjt(s),\vpubjt(s))$ respectively
for all agents $j$.
Here, recall, the former interval is obtained for agent $j$ when agent $i$ is being truthful
from the beginning
and the latter when $i$ is following $\pi^{t-1}_t$.
We now expand each term in the second summation as follows,
% Expanding each term in the second summation,
\begingroup
\allowdisplaybreaks
\begin{align*}
\numberthis
\label{eqn:opttruthsecondsum}
\utilitmot - \utilit \;&=\; \bigg(\vali(\sitmot) +
                                \Big(\valmech(\alltmot) + \sum_{j\neq i}\gpjt(\alltmot) \Big) -
                                \max_\alloc\Fpmit(\alloc) \bigg) \\
               &\hspace{1.0in}  - \bigg(\vali(\sit) +
                                \Big(\valmech(\alloct) + \sum_{j\neq i}\gjt(\alloct) \Big) -
                                \max_\alloc\Fmit(\alloc) \bigg), \\
%             &\hspace{0.4in} -   \bigg(\vali(\sitmot) +
%                                 \Big(\valmech(\alltmot) + \sum_{j\neq i}\gjt(\alltmot) \Big) -
%                                 \max_\alloc\Fmit(\alloc) \bigg), \\
%     &=\;  \vali(\sipit) - \vali(\sitmot) +
%                 \Big(\valmech(\allpit) + \sum_{j\neq i}\gjt(\allpit) \Big) -
%                 \Big(\valmech(\alltmot) + \sum_{j\neq i}\gjt(\alltmot) \Big), \\
    &=\;  \Big(\vali(\sitmot) - \gpit(\sitmot)\Big) + \Big(\git(\sit) - \vali(\sit)\Big) \\
       &\hspace{1in}     \,+\, 
            \Big(\Gpt(\alltmot) -\Gt(\alloct)\Big) + 
        \Big(\max_\alloc \Fmit(\alloc) -  \max_\alloc \Fpmit(\alloc)\big)\Big).
%         \\
%     &\leq\;(\vali(\sipit) - \git(\sipit)) + (\git(\sitmot) - \vali(\sitmot)).
\end{align*}
The first step uses the expressions in Fact~\ref{fac:algoutils}, while the second step
adds and subtracts $\gpit(\sitmot) + \git(\sit)$ and rearranges the terms.
To bound all four terms in~\eqref{eqn:opttruthsecondsum},
we will use that $\git$, $\gpit$, $\Gt$, $\Gpt$, $\Fmit$, $\Fpmit$ are all
computed under truthful reporting from agent $i$,
that all other agents are adopting stationary policies,
 and that  each agent has experienced each outcome at least
$\qt$ times~\eqref{eqn:qtdefn} in round $t$.
The first two terms are $0$ for an agent participating by bids.
If participating by rewards,
via a similar reasoning to that used in~\eqref{eqn:gdiffreasoning},
\[
\EE[(\vali(\sitmot) - \gpit(\sitmot)) + (\git(\sit) - \vali(\sit))|\Epit, \Eit]
\leq 2\sqrt{2} \sigma\betat \Kottmot.
\]
% This follows from the observation that when $g=\vub$,
% the first term is less than $0$ while the second is less than
% $2\betat\sigmait(\sit) \leq 2\sqrt{2} \sigma\betat \Kottmot$ by Lemma~\ref{lem:qTbound};
% a similar argument holds for $g=\vlb$, but with the terms reversed;
% when $g=\vbar$, both terms are less than $\sqrt{2} \sigma\betat \Kottmot$.
% 
%
% To bound the third term in~\eqref{eqn:opttruthsecondsum},
% % $\big(\Gpt(\alltmot) -\Gt(\alloct)\big)$.
% we first show that $\Gpt-\Gt$ is uniformly bounded under $\Et\cap\Ept$.
% Using the same reasoning about the $\git$ functions as~\eqref{eqn:gdiffreasoning},
% \begin{align*}
% \Gpt(\alloc) - \Gt(\alloc) = \sum_i (\gpit(\alloc) - \git(\alloc))
% = \sum_i (\gpit(\alloc) - \vali(\alloc)) + \sum_i(\vali(\alloc) - \git(\alloc))
% \leq 2\sqrt{2} \sigma\betat n \Kottmot.
% % = \sum_i (\vpbarit(\alloc) - \vbarit(\alloc)) + \sum_i \kappag(\sigmait(\alloc) + \sigmapit(\alloc))
% \end{align*}
% \endgroup
% In addition, under $\Et\cap\Ept$, we also have
% $\Vpubt(\alloc) - \Vubt(\alloc) \leq 2\sqrt{2} \sigma\betat n \Kottmot$.
To bound the third term in~\eqref{eqn:opttruthsecondsum},
% $\big(\Gpt(\alltmot) -\Gt(\alloct)\big)$.
observe that $\Vpubt-\Vubt$ is uniformly bounded under $\Et\cap\Ept$.
% Using the same reasoning about the $\git$ functions as~\eqref{eqn:gdiffreasoning},
\begin{align*}
\Vpubt(\alloc) - \Vubt(\alloc)
&= \sum_i (\vpubit(\alloc) - \vubit(\alloc))
= \sum_i (\vpubit(\alloc) - \vali(\alloc)) + \sum_i(\vali(\alloc) - \vubit(\alloc))
\\
&\leq 2\sqrt{2} \sigma\betat n \Kottmot.
% = \sum_i (\vpbarit(\alloc) - \vbarit(\alloc)) + \sum_i \kappag(\sigmait(\alloc) + \sigmapit(\alloc))
\end{align*}
\endgroup
% In addition, under $\Et\cap\Ept$, we also have
% $\Vpubt(\alloc) - \Vubt(\alloc) \leq 2\sqrt{2} \sigma\betat n \Kottmot$.
Observing that $\alltmot = \argmax_\alloc\Vpubt(\alloct)$ and
$\alloct = \argmax_\alloc\Vubt(\alloct)$, we use Lemma~\ref{lem:boundmax} to obtain,
\begin{align*}
\Gpt(\alltmot) - \Gt(\alloct)
&= \Vpubt(\alltmot) - \Vubt(\alloct) + \betat\kappag\sum_j(\sigmajt(\alloct) - \sigmapjt(\alltmot))
\\
&\leq (2+\kappag)\sqrt{2} \sigma\betat n \Kottmot.
\end{align*}
Here $\kappa_g=0$ if $g=\vlb$, $\kappa_g=1$ if $g=\vbar$, and $\kappa_g=2$ if $g=\vlb$.
Above,
the first step rewrites the expression for $\Gt, \Gpt$ in terms of
$\Vubt$,  $\Vpubt$, and $\kappag$.
The second step drops the $\sigmapit(\alltmot)$ terms and bounds the $\sigmait(\alltmot)$ terms
using Lemma~\ref{lem:qTbound}.
To bound the last term, we observe that $\Fpmit-\Fmit$ is uniformly bounded under $\Et\cap\Ept$.
Using a similar reasoning to~\eqref{eqn:gdiffreasoning},
\begin{align*}
\Fpt(\alloc) - \Ft(\alloc) &= \sum_i (\fpit(\alloc) - \fit(\alloc))
= \sum_i (\fpit(\alloc) - \vali(\alloc)) + \sum_i(\vali(\alloc) - \fit(\alloc))
\\
&\leq 2\sqrt{2} \sigma\betat n \Kottmot.
% = \sum_i (\vpbarit(\alloc) - \vbarit(\alloc)) + \sum_i \kappag(\sigmait(\alloc) + \sigmapit(\alloc))
\end{align*}
% By following an essentially similar argument, we can obtain the
% following bound on the last term in~\eqref{eqn:opttruthsecondsum} under $\Et\cap\Ept$.
By Lemma~\ref{lem:boundmax}, we therefore have,
% \begin{align*}
$
\max_\alloc \Fmit(\alloc) -  \max_\alloc \Fpmit(\alloc)
% &= \Vpubt(\alltmot) - \Vubt(\alloct) + \betat\kappag\sum_j(\sigmajt(\alloct) - \sigmapjt(\alltmot))
\leq 2\sqrt{2} \sigma\betat n \Kottmot.
$
% \end{align*}
Summing over all $t$ and using Lemma~\ref{lem:subounds}, we can now bound the second summation
in~\eqref{eqn:utildecomposition}.
\begin{align*}
\label{eqn:optsecondbound}
\numberthis
\sum_{t\notin\Expl} \EE[\utilitmot - \utilit | \Ept,\Et]
\leq
% \frac{3}{\sqrt{2}}\sigma \big(2\kappaiv + (8+\kappag)n\big) \betaT \KotTtt.
3\sqrt{2}\sigma \big(\kappaiv + n(4+\kappag/2)\big) \betaT \KotTtt.
\end{align*}
Finally,
we can combine the results in~\eqref{eqn:optfirstbound},~\eqref{eqn:optsecondbound} to
obtain
\begingroup
\allowdisplaybreaks
\begin{align*}
\EE[\UpiiT - \UiT] 
    &= \sum_{t\notin\Expl} \EE[\utilipit - \utilit]
    = \sum_{t\notin\Expl} \EE[\utilipit - \utilit|\Et,\Ept]
            + \sum_{t\notin\Expl}\PP(\Etc\cup\Eptc) \\
%     &= \sum_{t=1}^T \EE[\utilipit - \utilitmot]  + \sum_{t=2}^T \EE[\utilitmot - \utilit] \\
    &= \sum_{t\notin\Expl} \EE[\utilipit - \utilitmot|\Epit]  +
                    \sum_{t\notin\Expl} \EE[\utilitmot - \utilit|\Et,\Ept] + 12n \\
    &\leq 3\sqrt{2}\sigma \big(2\kappaiv + n(4+\kappag)\big) \betaT \KotTtt + 12n.
\end{align*}
\endgroup
The first step observes that the allocations and prices are the same during
the exploration phase rounds $\Expl$.
The third step uses Lemma~\ref{lem:Etcbound}, although it should be noted that $\Ept$
now refers to an event at each time step when the policy changes at each step.
% The last step uses the bounds in~\eqref{eqn:optfirstbound},~\eqref{eqn:optsecondbound}.
The claim follows by noting that $\kappag\leq 2$.
\qedwhite



==> vcgucb.tex <==


\section{An Optimistic Algorithm}
\label{sec:vcgucb}

Our second algorithm for this setting, called \vcgucbs (VCG-Upper-Confidence-Bound),
is outlined in Algorithm~\ref{alg:vcgucb}.
It operates similar to \vcgee, but with some important differences.
Each bracket begins with $K$ exploration rounds where the mechanism assigns all possible
outcomes to all customers, collects realised values, and does not charge them.
This is then followed by a phase where the algorithm chooses an optimistic allocation
by maximising an upper confidence bound on the welfare.
Crucially, it collects realised values on all rounds from the agents and uses them to determine
allocations and prices in future rounds.
Empirically, this is more desirable to \vcgee, as it uses samples collected on all rounds.
Theoretically, we show that the optimistic allocation provides flexible trade-offs in the
agent vs seller regrets~\eqref{eqn:regret}.
On the down side, this algorithm comes with weaker truthfulness guarantees than \vcgee.

\insertAlgoVCGUCB

To describe the algorithm, we define,
\begingroup
\allowdisplaybreaks
\begin{align*}
\label{eqn:ucbterms}
\numberthis
&\Nit(s) = \sum_{\ell=1}^{t-1} \indfone\big(\mapfuni(\allocl)=s), \\
&\vbarit(s) = \frac{1}{\Nit(s)}\sum_{\ell=1}^{t-1} \Xiitt{i}{\ell} \cdot
                \indfone\big(\mapfuni(\allocl)=s\big).
\end{align*}
\endgroup
Additionally,
$\vubit,\vlbit$ are defined as in~\eqref{eqn:eeterms}, but with the above definitions
for $\Nit,\vbarit$.
The key difference is that all samples, and not just those in the exploration phase,
are used in computing the confidence bounds.
For an agent $i$ who participates by bidding $\bidi$, we set
$\vbarit(s) = \vubit(s) = \vlbit(s) = \bidi(s)$ as in~\eqref{eqn:eebids}.
We also define $\Fit,\Vubt,\Vubmit$ as in~\eqref{eqn:eeqtys} but with the new
definitions for $\vubit,\vlbit$.
As before, $\Fit$ is decided by a parameter $f\in\{\vlb,\vub\}$ which determines if we wish to
price in a way that is favourable to the seller or agents.

\subsection*{Analysis}



